A Microscopic Pandemic Simulator for Pandemic Prediction Using Scalable Million-Agent Reinforcement Learning

Microscopic epidemic models are powerful tools for government policy makers to predict and simulate epidemic outbreaks, which can capture the impact of individual behaviors on the macroscopic phenomenon. However, existing models only consider simple rule-based individual behaviors, limiting their applicability. This paper proposes a deep-reinforcement-learning-powered microscopic model named Microscopic Pandemic Simulator (MPS). By replacing rule-based agents with rational agents whose behaviors are driven to maximize rewards, the MPS provides a better approximation of real world dynamics. To efficiently simulate with massive amounts of agents in MPS, we propose Scalable Million-Agent DQN (SMADQN). The MPS allows us to efficiently evaluate the impact of different government strategies. This paper first calibrates the MPS against real-world data in Allegheny, US, then demonstratively evaluates two government strategies: information disclosure and quarantine. The results validate the effectiveness of the proposed method. As a broad impact, this paper provides novel insights for the application of DRL in large scale agent-based networks such as economic and social networks.

==> pic/25M_rate_backup.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color2}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}

\begin{axis}[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black, fill=white!89.8039215686275!black},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={days},
xmajorgrids,
xmin=-3.95, xmax=82.95,
xtick style={color=white!33.3333333333333!black},
y grid style={white},
ylabel={cases},
ymajorgrids,
ymin=-10.6088647026423, ymax=307.055914768692,
ytick style={color=white!33.3333333333333!black}
]
\path [fill=color0, fill opacity=0.3, very thin]
(axis cs:0,11.3051678092668)
--(axis cs:0,5.49483219073321)
--(axis cs:1,11.3689011157193)
--(axis cs:2,9.9337634587642)
--(axis cs:3,18.8445670507415)
--(axis cs:4,22.661905976057)
--(axis cs:5,33.7607189753646)
--(axis cs:6,51.2724472470967)
--(axis cs:7,76.9529911726211)
--(axis cs:8,108.678072743174)
--(axis cs:9,149.602207559308)
--(axis cs:10,30.0731532816687)
--(axis cs:11,36.5714680415517)
--(axis cs:12,74.6274501002286)
--(axis cs:13,84.0767524184505)
--(axis cs:14,89.143329405043)
--(axis cs:15,96.1671061586828)
--(axis cs:16,98.4705980310559)
--(axis cs:17,93.8855632747791)
--(axis cs:18,99.0932452984681)
--(axis cs:19,95.1935910600805)
--(axis cs:20,90.8490614635103)
--(axis cs:21,84.4955734269414)
--(axis cs:22,86.9897462856066)
--(axis cs:23,94.3478816094677)
--(axis cs:24,86.9500943399585)
--(axis cs:25,84.4802010062941)
--(axis cs:26,84.1971225999795)
--(axis cs:27,78.426618436975)
--(axis cs:28,93.9350472426623)
--(axis cs:29,85.6977680795299)
--(axis cs:30,89.6558255891573)
--(axis cs:31,82.2597904202576)
--(axis cs:32,83.292386025583)
--(axis cs:33,80.1833415923377)
--(axis cs:34,80.7675666209117)
--(axis cs:35,88.3023974571165)
--(axis cs:36,92.3425647055055)
--(axis cs:37,80.1212565961726)
--(axis cs:38,86.8234834559363)
--(axis cs:39,81.964675354436)
--(axis cs:40,81.2997641522553)
--(axis cs:41,83.3739759700556)
--(axis cs:42,85.0864513122572)
--(axis cs:43,84.2837356369676)
--(axis cs:44,87.5542782624916)
--(axis cs:45,76.6741374088849)
--(axis cs:46,77.1098341772765)
--(axis cs:47,79.5097248492415)
--(axis cs:48,77.2011765112994)
--(axis cs:49,88.4970089293378)
--(axis cs:50,79.9833448913602)
--(axis cs:51,77.3429793741269)
--(axis cs:52,78.0953422886421)
--(axis cs:53,67.6853417035014)
--(axis cs:54,76.6625565327918)
--(axis cs:55,82.5675225522201)
--(axis cs:56,82.5056301887094)
--(axis cs:57,75.9923928768566)
--(axis cs:58,77.4911790133923)
--(axis cs:59,81.2418564164028)
--(axis cs:60,85.7474893582237)
--(axis cs:61,85.8565087837564)
--(axis cs:62,83.148860221857)
--(axis cs:63,84.9481373909534)
--(axis cs:64,83.7184338272928)
--(axis cs:65,83.7091271279001)
--(axis cs:66,82.8637105641053)
--(axis cs:67,86.2796804294982)
--(axis cs:68,79.0550758336864)
--(axis cs:69,89.248024189135)
--(axis cs:70,88.0655251810896)
--(axis cs:71,88.6147425616612)
--(axis cs:72,88.870296650387)
--(axis cs:73,87.1319933675024)
--(axis cs:74,91.4878338163166)
--(axis cs:75,91.467278300332)
--(axis cs:76,103.032479952582)
--(axis cs:77,87.9806924086104)
--(axis cs:78,99.7300392328483)
--(axis cs:79,94.8142000529517)
--(axis cs:79,125.785799947048)
--(axis cs:79,125.785799947048)
--(axis cs:78,122.669960767152)
--(axis cs:77,123.21930759139)
--(axis cs:76,125.167520047418)
--(axis cs:75,120.532721699668)
--(axis cs:74,121.912166183683)
--(axis cs:73,113.668006632498)
--(axis cs:72,112.129703349613)
--(axis cs:71,126.585257438339)
--(axis cs:70,107.53447481891)
--(axis cs:69,118.351975810865)
--(axis cs:68,118.944924166314)
--(axis cs:67,116.320319570502)
--(axis cs:66,112.936289435895)
--(axis cs:65,111.0908728721)
--(axis cs:64,110.281566172707)
--(axis cs:63,110.451862609047)
--(axis cs:62,116.051139778143)
--(axis cs:61,107.743491216244)
--(axis cs:60,108.652510641776)
--(axis cs:59,107.958143583597)
--(axis cs:58,108.108820986608)
--(axis cs:57,112.807607123143)
--(axis cs:56,112.694369811291)
--(axis cs:55,107.23247744778)
--(axis cs:54,101.537443467208)
--(axis cs:53,109.314658296499)
--(axis cs:52,110.304657711358)
--(axis cs:51,104.057020625873)
--(axis cs:50,104.01665510864)
--(axis cs:49,111.902991070662)
--(axis cs:48,111.198823488701)
--(axis cs:47,115.490275150759)
--(axis cs:46,112.690165822724)
--(axis cs:45,116.525862591115)
--(axis cs:44,113.845721737508)
--(axis cs:43,118.116264363032)
--(axis cs:42,118.313548687743)
--(axis cs:41,121.826024029944)
--(axis cs:40,123.700235847745)
--(axis cs:39,118.235324645564)
--(axis cs:38,125.976516544064)
--(axis cs:37,110.678743403827)
--(axis cs:36,120.257435294494)
--(axis cs:35,117.497602542884)
--(axis cs:34,111.632433379088)
--(axis cs:33,113.816658407662)
--(axis cs:32,113.507613974417)
--(axis cs:31,122.340209579742)
--(axis cs:30,117.544174410843)
--(axis cs:29,108.10223192047)
--(axis cs:28,119.864952757338)
--(axis cs:27,118.973381563025)
--(axis cs:26,112.00287740002)
--(axis cs:25,116.319798993706)
--(axis cs:24,113.449905660042)
--(axis cs:23,112.052118390532)
--(axis cs:22,126.010253714393)
--(axis cs:21,122.904426573059)
--(axis cs:20,120.15093853649)
--(axis cs:19,126.40640893992)
--(axis cs:18,121.306754701532)
--(axis cs:17,120.914436725221)
--(axis cs:16,126.729401968944)
--(axis cs:15,129.032893841317)
--(axis cs:14,120.256670594957)
--(axis cs:13,121.52324758155)
--(axis cs:12,109.572549899771)
--(axis cs:11,202.028531958448)
--(axis cs:10,170.526846718331)
--(axis cs:9,240.197792440692)
--(axis cs:8,159.321927256826)
--(axis cs:7,121.247008827379)
--(axis cs:6,84.3275527529032)
--(axis cs:5,58.2392810246354)
--(axis cs:4,41.338094023943)
--(axis cs:3,34.9554329492585)
--(axis cs:2,20.2662365412358)
--(axis cs:1,17.8310988842807)
--(axis cs:0,11.3051678092668)
--cycle;

\path [fill=color1, fill opacity=0.3, very thin]
(axis cs:0,10.3695565448544)
--(axis cs:0,3.83044345514564)
--(axis cs:1,10.015415080089)
--(axis cs:2,11.1423588545111)
--(axis cs:3,12.9937530487812)
--(axis cs:4,18.9875097503959)
--(axis cs:5,29.2812017942226)
--(axis cs:6,41.0716117228159)
--(axis cs:7,62.2061548174815)
--(axis cs:8,84.6547649401425)
--(axis cs:9,125.146816280577)
--(axis cs:10,150.401733128282)
--(axis cs:11,56.9589796661372)
--(axis cs:12,80.6269580160881)
--(axis cs:13,81.2851322054354)
--(axis cs:14,91.6579902009673)
--(axis cs:15,103.849556224671)
--(axis cs:16,102.429519547563)
--(axis cs:17,96.0891834700493)
--(axis cs:18,96.5445866039105)
--(axis cs:19,101.16349588721)
--(axis cs:20,95.6663148685746)
--(axis cs:21,95.5811868803961)
--(axis cs:22,113.497852902148)
--(axis cs:23,113.202353266933)
--(axis cs:24,115.511228778417)
--(axis cs:25,110.950103734886)
--(axis cs:26,109.263877510511)
--(axis cs:27,115.821599515794)
--(axis cs:28,120.5338572445)
--(axis cs:29,127.381666793874)
--(axis cs:30,128.398333449058)
--(axis cs:31,132.492859570749)
--(axis cs:32,139.25622247508)
--(axis cs:33,131.613705062628)
--(axis cs:34,141.912854327891)
--(axis cs:35,147.986672587331)
--(axis cs:36,150.650818206162)
--(axis cs:37,147.819131102908)
--(axis cs:38,144.050722573533)
--(axis cs:39,134.231979955471)
--(axis cs:40,139.673195708948)
--(axis cs:41,128.917839924474)
--(axis cs:42,120.368852168559)
--(axis cs:43,131.882883933321)
--(axis cs:44,138.81176979883)
--(axis cs:45,143.021081871401)
--(axis cs:46,125.808165533195)
--(axis cs:47,130.471139126149)
--(axis cs:48,142.562331082422)
--(axis cs:49,133.32685095335)
--(axis cs:50,136.501388978207)
--(axis cs:51,136.779613042247)
--(axis cs:52,129.896602502087)
--(axis cs:53,134.398795224442)
--(axis cs:54,141.413611744203)
--(axis cs:55,137.917171316378)
--(axis cs:56,136.196491767881)
--(axis cs:57,134.398461629484)
--(axis cs:58,132.320859232594)
--(axis cs:59,124.97067554141)
--(axis cs:60,119.785427726622)
--(axis cs:61,113.95344072901)
--(axis cs:62,115.56157395579)
--(axis cs:63,121.97553056983)
--(axis cs:64,131.838532922409)
--(axis cs:65,132.100322584002)
--(axis cs:66,121.213611744203)
--(axis cs:67,124.453700165526)
--(axis cs:68,131.454858938829)
--(axis cs:69,119.932614959212)
--(axis cs:70,124.266799469318)
--(axis cs:71,131.292427138799)
--(axis cs:72,127.878120219764)
--(axis cs:73,125.098310907197)
--(axis cs:74,135.773714514331)
--(axis cs:75,133.808853025489)
--(axis cs:76,136.003252462541)
--(axis cs:77,125.240051746529)
--(axis cs:78,131.465794096215)
--(axis cs:79,138.641789437305)
--(axis cs:79,166.358210562695)
--(axis cs:79,166.358210562695)
--(axis cs:78,156.934205903785)
--(axis cs:77,156.159948253471)
--(axis cs:76,160.596747537459)
--(axis cs:75,156.391146974511)
--(axis cs:74,158.626285485669)
--(axis cs:73,154.701689092803)
--(axis cs:72,158.521879780236)
--(axis cs:71,151.107572861201)
--(axis cs:70,157.733200530682)
--(axis cs:69,150.867385040788)
--(axis cs:68,152.545141061171)
--(axis cs:67,146.746299834474)
--(axis cs:66,150.586388255797)
--(axis cs:65,163.099677415998)
--(axis cs:64,152.561467077591)
--(axis cs:63,151.42446943017)
--(axis cs:62,157.23842604421)
--(axis cs:61,146.64655927099)
--(axis cs:60,139.014572273378)
--(axis cs:59,161.82932445859)
--(axis cs:58,149.079140767406)
--(axis cs:57,160.401538370516)
--(axis cs:56,159.003508232119)
--(axis cs:55,158.282828683622)
--(axis cs:54,170.786388255797)
--(axis cs:53,167.601204775558)
--(axis cs:52,150.503397497913)
--(axis cs:51,156.420386957753)
--(axis cs:50,158.098611021794)
--(axis cs:49,155.27314904665)
--(axis cs:48,163.837668917578)
--(axis cs:47,152.328860873851)
--(axis cs:46,155.191834466805)
--(axis cs:45,158.178918128599)
--(axis cs:44,165.98823020117)
--(axis cs:43,153.517116066679)
--(axis cs:42,166.631147831441)
--(axis cs:41,151.882160075526)
--(axis cs:40,158.726804291052)
--(axis cs:39,162.968020044529)
--(axis cs:38,161.349277426467)
--(axis cs:37,174.980868897092)
--(axis cs:36,178.149181793838)
--(axis cs:35,178.013327412669)
--(axis cs:34,184.687145672109)
--(axis cs:33,160.786294937372)
--(axis cs:32,160.54377752492)
--(axis cs:31,153.507140429251)
--(axis cs:30,152.401666550942)
--(axis cs:29,149.218333206126)
--(axis cs:28,154.4661427555)
--(axis cs:27,143.578400484206)
--(axis cs:26,141.136122489489)
--(axis cs:25,135.049896265114)
--(axis cs:24,144.888771221583)
--(axis cs:23,130.197646733067)
--(axis cs:22,146.102147097852)
--(axis cs:21,129.618813119604)
--(axis cs:20,120.933685131425)
--(axis cs:19,117.63650411279)
--(axis cs:18,118.25541339609)
--(axis cs:17,122.910816529951)
--(axis cs:16,121.370480452437)
--(axis cs:15,120.750443775329)
--(axis cs:14,115.742009799033)
--(axis cs:13,98.1148677945646)
--(axis cs:12,101.373041983912)
--(axis cs:11,180.841020333863)
--(axis cs:10,265.798266871718)
--(axis cs:9,215.453183719423)
--(axis cs:8,131.345235059858)
--(axis cs:7,101.193845182519)
--(axis cs:6,68.9283882771841)
--(axis cs:5,47.9187982057774)
--(axis cs:4,35.0124902496041)
--(axis cs:3,25.8062469512188)
--(axis cs:2,16.0576411454889)
--(axis cs:1,17.784584919911)
--(axis cs:0,10.3695565448544)
--cycle;

\path [fill=color2, fill opacity=0.3, very thin]
(axis cs:0,9.04899959967968)
--(axis cs:0,6.55100040032032)
--(axis cs:1,9.55672529350244)
--(axis cs:2,9.2)
--(axis cs:3,12.9037323828867)
--(axis cs:4,21.7461419385663)
--(axis cs:5,33.6735587872995)
--(axis cs:6,42.6290160119184)
--(axis cs:7,61.8861545269267)
--(axis cs:8,91.5992424351118)
--(axis cs:9,132.683907066011)
--(axis cs:10,149.75106597857)
--(axis cs:11,20.4595544079182)
--(axis cs:12,80.2981885246899)
--(axis cs:13,83.9378635763366)
--(axis cs:14,106.006731858604)
--(axis cs:15,117.206385147346)
--(axis cs:16,113.137976759762)
--(axis cs:17,110.561953996544)
--(axis cs:18,119.306029658042)
--(axis cs:19,111.761490451366)
--(axis cs:20,105.260423512951)
--(axis cs:21,115.888864455454)
--(axis cs:22,124.216892381576)
--(axis cs:23,121.648839719251)
--(axis cs:24,127.778479351474)
--(axis cs:25,116.525861369478)
--(axis cs:26,128.454224871178)
--(axis cs:27,131.838248315164)
--(axis cs:28,124.961459020485)
--(axis cs:29,134.246798644378)
--(axis cs:30,130.732502103984)
--(axis cs:31,137.259060350433)
--(axis cs:32,144.069383837237)
--(axis cs:33,155.733490196947)
--(axis cs:34,158.657338554154)
--(axis cs:35,164.751570167412)
--(axis cs:36,148.52602709639)
--(axis cs:37,132.611699909002)
--(axis cs:38,130.947286544177)
--(axis cs:39,131.873181633596)
--(axis cs:40,130.81260838175)
--(axis cs:41,142.429005829424)
--(axis cs:42,144.084813001241)
--(axis cs:43,145.672517166049)
--(axis cs:44,149.666420211173)
--(axis cs:45,149.745732200924)
--(axis cs:46,150.838363995754)
--(axis cs:47,159.236184014545)
--(axis cs:48,157.191718005664)
--(axis cs:49,169.497976996894)
--(axis cs:50,162.8)
--(axis cs:51,181.221965929941)
--(axis cs:52,177.504412337315)
--(axis cs:53,187.934699510922)
--(axis cs:54,185.818509749137)
--(axis cs:55,187.13910238883)
--(axis cs:56,190.956229993612)
--(axis cs:57,172.690855358221)
--(axis cs:58,182.228455206132)
--(axis cs:59,180.942934677406)
--(axis cs:60,169.044177268334)
--(axis cs:61,173.094974213189)
--(axis cs:62,177.824678391198)
--(axis cs:63,167.614222803036)
--(axis cs:64,159.225577474534)
--(axis cs:65,164.838753997974)
--(axis cs:66,157.408590088798)
--(axis cs:67,160.695915305306)
--(axis cs:68,163.444612853044)
--(axis cs:69,171.739338314022)
--(axis cs:70,173.632697207637)
--(axis cs:71,167.991420356605)
--(axis cs:72,172.221762694998)
--(axis cs:73,175.63583035557)
--(axis cs:74,165.882243511834)
--(axis cs:75,181.48542523738)
--(axis cs:76,171.111395842697)
--(axis cs:77,179.503154970878)
--(axis cs:78,186.748945055083)
--(axis cs:79,176.983393389096)
--(axis cs:79,292.616606610904)
--(axis cs:79,292.616606610904)
--(axis cs:78,288.651054944917)
--(axis cs:77,284.096845029122)
--(axis cs:76,245.688604157303)
--(axis cs:75,254.91457476262)
--(axis cs:74,232.917756488166)
--(axis cs:73,248.16416964443)
--(axis cs:72,229.178237305002)
--(axis cs:71,228.608579643395)
--(axis cs:70,234.767302792363)
--(axis cs:69,214.660661685978)
--(axis cs:68,227.955387146956)
--(axis cs:67,221.904084694694)
--(axis cs:66,222.591409911202)
--(axis cs:65,227.761246002026)
--(axis cs:64,229.574422525466)
--(axis cs:63,209.785777196964)
--(axis cs:62,206.975321608802)
--(axis cs:61,210.905025786811)
--(axis cs:60,211.555822731666)
--(axis cs:59,223.057065322594)
--(axis cs:58,224.371544793868)
--(axis cs:57,221.909144641779)
--(axis cs:56,220.243770006388)
--(axis cs:55,241.06089761117)
--(axis cs:54,231.181490250863)
--(axis cs:53,220.465300489078)
--(axis cs:52,211.495587662685)
--(axis cs:51,213.978034070059)
--(axis cs:50,211.6)
--(axis cs:49,204.102023003106)
--(axis cs:48,191.008281994336)
--(axis cs:47,192.363815985455)
--(axis cs:46,198.761636004246)
--(axis cs:45,186.654267799076)
--(axis cs:44,185.733579788827)
--(axis cs:43,189.727482833951)
--(axis cs:42,180.315186998759)
--(axis cs:41,183.770994170576)
--(axis cs:40,178.38739161825)
--(axis cs:39,175.526818366404)
--(axis cs:38,174.252713455823)
--(axis cs:37,166.788300090998)
--(axis cs:36,173.47397290361)
--(axis cs:35,185.448429832588)
--(axis cs:34,175.342661445846)
--(axis cs:33,184.066509803053)
--(axis cs:32,165.330616162763)
--(axis cs:31,171.740939649567)
--(axis cs:30,157.467497896016)
--(axis cs:29,170.953201355622)
--(axis cs:28,164.438540979515)
--(axis cs:27,153.761751684836)
--(axis cs:26,164.545775128822)
--(axis cs:25,146.274138630522)
--(axis cs:24,153.821520648526)
--(axis cs:23,145.351160280749)
--(axis cs:22,154.983107618424)
--(axis cs:21,156.311135544546)
--(axis cs:20,151.539576487049)
--(axis cs:19,145.038509548634)
--(axis cs:18,147.493970341958)
--(axis cs:17,140.038046003456)
--(axis cs:16,137.062023240238)
--(axis cs:15,135.993614852654)
--(axis cs:14,147.593268141396)
--(axis cs:13,129.062136423663)
--(axis cs:12,107.90181147531)
--(axis cs:11,182.940445592082)
--(axis cs:10,274.04893402143)
--(axis cs:9,220.316092933989)
--(axis cs:8,144.400757564888)
--(axis cs:7,117.513845473073)
--(axis cs:6,70.1709839880816)
--(axis cs:5,57.5264412127005)
--(axis cs:4,36.6538580614337)
--(axis cs:3,26.2962676171133)
--(axis cs:2,19.6)
--(axis cs:1,18.8432747064976)
--(axis cs:0,9.04899959967968)
--cycle;

\addplot [semithick, color0]
table {%
0 8.4
1 14.6
2 15.1
3 26.9
4 32
5 46
6 67.8
7 99.1
8 134
9 194.9
10 100.3
11 119.3
12 92.1
13 102.8
14 104.7
15 112.6
16 112.6
17 107.4
18 110.2
19 110.8
20 105.5
21 103.7
22 106.5
23 103.2
24 100.2
25 100.4
26 98.1
27 98.7
28 106.9
29 96.9
30 103.6
31 102.3
32 98.4
33 97
34 96.2
35 102.9
36 106.3
37 95.4
38 106.4
39 100.1
40 102.5
41 102.6
42 101.7
43 101.2
44 100.7
45 96.6
46 94.9
47 97.5
48 94.2
49 100.2
50 92
51 90.7
52 94.2
53 88.5
54 89.1
55 94.9
56 97.6
57 94.4
58 92.8
59 94.6
60 97.2
61 96.8
62 99.6
63 97.7
64 97
65 97.4
66 97.9
67 101.3
68 99
69 103.8
70 97.8
71 107.6
72 100.5
73 100.4
74 106.7
75 106
76 114.1
77 105.6
78 111.2
79 110.3
};
\addlegendentry{-0.1}
\addplot [semithick, color1]
table {%
0 7.1
1 13.9
2 13.6
3 19.4
4 27
5 38.6
6 55
7 81.7
8 108
9 170.3
10 208.1
11 118.9
12 91
13 89.7
14 103.7
15 112.3
16 111.9
17 109.5
18 107.4
19 109.4
20 108.3
21 112.6
22 129.8
23 121.7
24 130.2
25 123
26 125.2
27 129.7
28 137.5
29 138.3
30 140.4
31 143
32 149.9
33 146.2
34 163.3
35 163
36 164.4
37 161.4
38 152.7
39 148.6
40 149.2
41 140.4
42 143.5
43 142.7
44 152.4
45 150.6
46 140.5
47 141.4
48 153.2
49 144.3
50 147.3
51 146.6
52 140.2
53 151
54 156.1
55 148.1
56 147.6
57 147.4
58 140.7
59 143.4
60 129.4
61 130.3
62 136.4
63 136.7
64 142.2
65 147.6
66 135.9
67 135.6
68 142
69 135.4
70 141
71 141.2
72 143.2
73 139.9
74 147.2
75 145.1
76 148.3
77 140.7
78 144.2
79 152.5
};
\addlegendentry{-0.3}
\addplot [semithick, color2]
table {%
0 7.8
1 14.2
2 14.4
3 19.6
4 29.2
5 45.6
6 56.4
7 89.7
8 118
9 176.5
10 211.9
11 101.7
12 94.1
13 106.5
14 126.8
15 126.6
16 125.1
17 125.3
18 133.4
19 128.4
20 128.4
21 136.1
22 139.6
23 133.5
24 140.8
25 131.4
26 146.5
27 142.8
28 144.7
29 152.6
30 144.1
31 154.5
32 154.7
33 169.9
34 167
35 175.1
36 161
37 149.7
38 152.6
39 153.7
40 154.6
41 163.1
42 162.2
43 167.7
44 167.7
45 168.2
46 174.8
47 175.8
48 174.1
49 186.8
50 187.2
51 197.6
52 194.5
53 204.2
54 208.5
55 214.1
56 205.6
57 197.3
58 203.3
59 202
60 190.3
61 192
62 192.4
63 188.7
64 194.4
65 196.3
66 190
67 191.3
68 195.7
69 193.2
70 204.2
71 198.3
72 200.7
73 211.9
74 199.4
75 218.2
76 208.4
77 231.8
78 237.7
79 234.8
};
\addlegendentry{-0.5}
\end{axis}

\end{tikzpicture}


==> pic/25beta_backup.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color2}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}

\begin{axis}[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=white!89.8039215686275!black},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={days},
xmajorgrids,
xmin=-3.95, xmax=82.95,
xtick style={color=white!33.3333333333333!black},
y grid style={white},
ylabel={cases},
ymajorgrids,
ymin=-73.626372730155, ymax=849.626372730155,
ytick style={color=white!33.3333333333333!black}
]
\path [fill=color0, fill opacity=0.3, very thin]
(axis cs:0,6.0976176963403)
--(axis cs:0,1.9023823036597)
--(axis cs:1,4.29108561896237)
--(axis cs:2,3.93012968542051)
--(axis cs:3,8.91197210121821)
--(axis cs:4,10.1642662691691)
--(axis cs:5,10.5352384841238)
--(axis cs:6,17.6955374923192)
--(axis cs:7,17.0081125549695)
--(axis cs:8,29.1319387552555)
--(axis cs:9,41.2931214364512)
--(axis cs:10,54.1273364338699)
--(axis cs:11,57.7982684631649)
--(axis cs:12,87.9464115055302)
--(axis cs:13,97.3338230188145)
--(axis cs:14,38.3923780226365)
--(axis cs:15,31.3446752577704)
--(axis cs:16,43.4907655041258)
--(axis cs:17,51.5590191391068)
--(axis cs:18,51.0784237983012)
--(axis cs:19,48.6932452984681)
--(axis cs:20,54.1007246757359)
--(axis cs:21,44.2772509732344)
--(axis cs:22,53.8179344510848)
--(axis cs:23,47.1671224080033)
--(axis cs:24,45.09263775979)
--(axis cs:25,48.0670833496106)
--(axis cs:26,43.2024099884364)
--(axis cs:27,49.9151429428743)
--(axis cs:28,45.4)
--(axis cs:29,42.9863327689404)
--(axis cs:30,44.9761618103943)
--(axis cs:31,45.5250333333926)
--(axis cs:32,42.8419628418661)
--(axis cs:33,46.9427276659705)
--(axis cs:34,45.7307895450093)
--(axis cs:35,37.5323970406826)
--(axis cs:36,38.9302432998607)
--(axis cs:37,41.6803800560833)
--(axis cs:38,39.9857288332999)
--(axis cs:39,39.3917854437626)
--(axis cs:40,39.4369318395244)
--(axis cs:41,31.6258909630158)
--(axis cs:42,42.9934461436912)
--(axis cs:43,39.4100062578247)
--(axis cs:44,36.8026671409094)
--(axis cs:45,38.0971595493273)
--(axis cs:46,38.5140364036969)
--(axis cs:47,32.4612040202497)
--(axis cs:48,32.0408178749498)
--(axis cs:49,35.203334259774)
--(axis cs:50,37.052372673692)
--(axis cs:51,33.7564309346812)
--(axis cs:52,37.4103147625942)
--(axis cs:53,33.9470936780393)
--(axis cs:54,35.9006666962989)
--(axis cs:55,35.1281015150586)
--(axis cs:56,34.0858069002319)
--(axis cs:57,35.5347749432807)
--(axis cs:58,34.5155563866035)
--(axis cs:59,35.809844008566)
--(axis cs:60,37.1959604201114)
--(axis cs:61,36.6)
--(axis cs:62,34.8868260705644)
--(axis cs:63,36.9541958124055)
--(axis cs:64,31.8977680795299)
--(axis cs:65,31.5768097227214)
--(axis cs:66,37.7558385060861)
--(axis cs:67,39.3770417861829)
--(axis cs:68,36.2830236987769)
--(axis cs:69,36.356349239007)
--(axis cs:70,33.6568010985331)
--(axis cs:71,36.9688518443852)
--(axis cs:72,39.7297971376751)
--(axis cs:73,34.7330363800803)
--(axis cs:74,35.2719168244009)
--(axis cs:75,41.2695498865613)
--(axis cs:76,39.9487374274104)
--(axis cs:77,39.255852104776)
--(axis cs:78,42.7657561657209)
--(axis cs:79,37.201190518373)
--(axis cs:79,70.798809481627)
--(axis cs:79,70.798809481627)
--(axis cs:78,70.8342438342791)
--(axis cs:77,72.144147895224)
--(axis cs:76,69.6512625725896)
--(axis cs:75,65.9304501134387)
--(axis cs:74,69.1280831755991)
--(axis cs:73,64.6669636199197)
--(axis cs:72,64.8702028623248)
--(axis cs:71,58.8311481556148)
--(axis cs:70,57.5431989014669)
--(axis cs:69,55.643650760993)
--(axis cs:68,56.9169763012231)
--(axis cs:67,56.8229582138171)
--(axis cs:66,60.444161493914)
--(axis cs:65,54.0231902772786)
--(axis cs:64,54.3022319204701)
--(axis cs:63,51.8458041875945)
--(axis cs:62,56.9131739294356)
--(axis cs:61,56.8)
--(axis cs:60,57.0040395798886)
--(axis cs:59,47.990155991434)
--(axis cs:58,58.2844436133965)
--(axis cs:57,47.8652250567193)
--(axis cs:56,51.7141930997681)
--(axis cs:55,54.6718984849414)
--(axis cs:54,50.8993333037011)
--(axis cs:53,46.8529063219607)
--(axis cs:52,56.7896852374058)
--(axis cs:51,51.2435690653188)
--(axis cs:50,50.747627326308)
--(axis cs:49,47.196665740226)
--(axis cs:48,53.5591821250502)
--(axis cs:47,48.7387959797503)
--(axis cs:46,54.8859635963031)
--(axis cs:45,55.7028404506727)
--(axis cs:44,51.7973328590906)
--(axis cs:43,55.3899937421753)
--(axis cs:42,55.2065538563088)
--(axis cs:41,54.7741090369842)
--(axis cs:40,54.5630681604756)
--(axis cs:39,54.0082145562374)
--(axis cs:38,54.0142711667001)
--(axis cs:37,58.5196199439167)
--(axis cs:36,59.0697567001393)
--(axis cs:35,61.2676029593174)
--(axis cs:34,54.4692104549907)
--(axis cs:33,65.8572723340295)
--(axis cs:32,59.9580371581339)
--(axis cs:31,64.2749666666074)
--(axis cs:30,58.4238381896057)
--(axis cs:29,66.4136672310596)
--(axis cs:28,59.2)
--(axis cs:27,58.4848570571257)
--(axis cs:26,59.7975900115636)
--(axis cs:25,58.7329166503894)
--(axis cs:24,70.90736224021)
--(axis cs:23,64.2328775919967)
--(axis cs:22,67.1820655489152)
--(axis cs:21,62.3227490267656)
--(axis cs:20,67.8992753242641)
--(axis cs:19,70.9067547015319)
--(axis cs:18,67.3215762016988)
--(axis cs:17,66.2409808608932)
--(axis cs:16,61.9092344958742)
--(axis cs:15,92.8553247422296)
--(axis cs:14,148.607621977364)
--(axis cs:13,160.866176981186)
--(axis cs:12,129.05358849447)
--(axis cs:11,104.001731536835)
--(axis cs:10,80.0726635661301)
--(axis cs:9,63.1068785635488)
--(axis cs:8,45.0680612447445)
--(axis cs:7,31.7918874450305)
--(axis cs:6,28.9044625076808)
--(axis cs:5,19.8647615158762)
--(axis cs:4,18.0357337308309)
--(axis cs:3,18.0880278987818)
--(axis cs:2,10.8698703145795)
--(axis cs:1,9.90891438103763)
--(axis cs:0,6.0976176963403)
--cycle;

\path [fill=color1, fill opacity=0.3, very thin]
(axis cs:0,8.93830292855994)
--(axis cs:0,4.46169707144006)
--(axis cs:1,8.28840486136072)
--(axis cs:2,13.5046909382659)
--(axis cs:3,14.4589199622371)
--(axis cs:4,20.1417990271722)
--(axis cs:5,31.8156441201951)
--(axis cs:6,44.9077723111088)
--(axis cs:7,68.8972893779359)
--(axis cs:8,98.0152591703873)
--(axis cs:9,130.856342821898)
--(axis cs:10,121.072566074663)
--(axis cs:11,29.7965184924651)
--(axis cs:12,70.7397192539712)
--(axis cs:13,83.504696741972)
--(axis cs:14,91.0274694748051)
--(axis cs:15,89.8838290231196)
--(axis cs:16,94.8240989727877)
--(axis cs:17,86.9794195506415)
--(axis cs:18,91.5766817705507)
--(axis cs:19,85.0236659512051)
--(axis cs:20,91.9503602342873)
--(axis cs:21,80.2742809184107)
--(axis cs:22,78.1324062531296)
--(axis cs:23,85.3393568856745)
--(axis cs:24,78.0450793756573)
--(axis cs:25,84.1314336462837)
--(axis cs:26,81.1089306060134)
--(axis cs:27,87.3488318182134)
--(axis cs:28,83.7958978673716)
--(axis cs:29,84.7334358976787)
--(axis cs:30,80.8735710775099)
--(axis cs:31,84.6675438813457)
--(axis cs:32,78.900276245202)
--(axis cs:33,78.3090377847702)
--(axis cs:34,90.7367327412384)
--(axis cs:35,74.8375258858844)
--(axis cs:36,81.255333197867)
--(axis cs:37,93.3182201226194)
--(axis cs:38,84.6860455514374)
--(axis cs:39,90.511643774892)
--(axis cs:40,80.8069274456602)
--(axis cs:41,82.2099034177645)
--(axis cs:42,82.7398935143112)
--(axis cs:43,90.2620088163057)
--(axis cs:44,82.2030153038205)
--(axis cs:45,80.7120725553348)
--(axis cs:46,79.8772850710048)
--(axis cs:47,82.5112287784172)
--(axis cs:48,86.7681121498667)
--(axis cs:49,80.6996875030517)
--(axis cs:50,79.0365008926842)
--(axis cs:51,73.0742301364544)
--(axis cs:52,79.5443062709865)
--(axis cs:53,79.9327316584179)
--(axis cs:54,75.686013660956)
--(axis cs:55,75.4410145238303)
--(axis cs:56,79.5136420031591)
--(axis cs:57,79.170086670876)
--(axis cs:58,80.1192129078495)
--(axis cs:59,85.1719992542879)
--(axis cs:60,78.798190119359)
--(axis cs:61,76.5628027562485)
--(axis cs:62,86.2512108679829)
--(axis cs:63,80.5269416885791)
--(axis cs:64,85.6788740371244)
--(axis cs:65,90.587884348069)
--(axis cs:66,87.2811837669946)
--(axis cs:67,86.5207422009488)
--(axis cs:68,85.7060138027159)
--(axis cs:69,92.3848355159165)
--(axis cs:70,86.5990867770314)
--(axis cs:71,91.2718343347631)
--(axis cs:72,87.8264963992343)
--(axis cs:73,98.649688800699)
--(axis cs:74,89.5907427244711)
--(axis cs:75,90.7910910734894)
--(axis cs:76,97.5166747967499)
--(axis cs:77,83.5715507370891)
--(axis cs:78,87.7686055386571)
--(axis cs:79,88.3421360353673)
--(axis cs:79,163.057863964633)
--(axis cs:79,163.057863964633)
--(axis cs:78,150.231394461343)
--(axis cs:77,137.028449262911)
--(axis cs:76,131.68332520325)
--(axis cs:75,131.208908926511)
--(axis cs:74,132.809257275529)
--(axis cs:73,122.750311199301)
--(axis cs:72,114.973503600766)
--(axis cs:71,117.928165665237)
--(axis cs:70,130.400913222969)
--(axis cs:69,121.415164484084)
--(axis cs:68,117.293986197284)
--(axis cs:67,127.479257799051)
--(axis cs:66,119.718816233005)
--(axis cs:65,117.012115651931)
--(axis cs:64,115.521125962876)
--(axis cs:63,119.473058311421)
--(axis cs:62,121.348789132017)
--(axis cs:61,114.237197243752)
--(axis cs:60,123.001809880641)
--(axis cs:59,106.628000745712)
--(axis cs:58,102.480787092151)
--(axis cs:57,112.629913329124)
--(axis cs:56,112.486357996841)
--(axis cs:55,108.55898547617)
--(axis cs:54,119.313986339044)
--(axis cs:53,116.867268341582)
--(axis cs:52,105.455693729014)
--(axis cs:51,117.725769863546)
--(axis cs:50,115.163499107316)
--(axis cs:49,112.700312496948)
--(axis cs:48,124.431887850133)
--(axis cs:47,111.888771221583)
--(axis cs:46,121.722714928995)
--(axis cs:45,121.287927444665)
--(axis cs:44,121.996984696179)
--(axis cs:43,117.937991183694)
--(axis cs:42,124.060106485689)
--(axis cs:41,122.590096582236)
--(axis cs:40,126.99307255434)
--(axis cs:39,113.688356225108)
--(axis cs:38,124.113954448563)
--(axis cs:37,125.681779877381)
--(axis cs:36,117.344666802133)
--(axis cs:35,129.162474114116)
--(axis cs:34,131.263267258762)
--(axis cs:33,128.09096221523)
--(axis cs:32,115.099723754798)
--(axis cs:31,120.132456118654)
--(axis cs:30,125.92642892249)
--(axis cs:29,128.066564102321)
--(axis cs:28,122.804102132628)
--(axis cs:27,119.451168181787)
--(axis cs:26,120.291069393987)
--(axis cs:25,109.868566353716)
--(axis cs:24,116.154920624343)
--(axis cs:23,117.060643114325)
--(axis cs:22,130.86759374687)
--(axis cs:21,121.125719081589)
--(axis cs:20,126.649639765713)
--(axis cs:19,140.776334048795)
--(axis cs:18,127.623318229449)
--(axis cs:17,141.420580449359)
--(axis cs:16,132.975901027212)
--(axis cs:15,137.51617097688)
--(axis cs:14,131.772530525195)
--(axis cs:13,119.695303258028)
--(axis cs:12,100.660280746029)
--(axis cs:11,133.203481507535)
--(axis cs:10,268.727433925337)
--(axis cs:9,205.343657178102)
--(axis cs:8,145.184740829613)
--(axis cs:7,102.102710622064)
--(axis cs:6,74.4922276888912)
--(axis cs:5,44.584355879805)
--(axis cs:4,33.2582009728278)
--(axis cs:3,25.9410800377629)
--(axis cs:2,19.8953090617341)
--(axis cs:1,19.5115951386393)
--(axis cs:0,8.93830292855994)
--cycle;

\path [fill=color2, fill opacity=0.3, very thin]
(axis cs:0,11.3518284528683)
--(axis cs:0,7.24817154713168)
--(axis cs:1,9.56239754196699)
--(axis cs:2,17.7477279431484)
--(axis cs:3,21.8866323024885)
--(axis cs:4,31.3201930047422)
--(axis cs:5,50.9562695961013)
--(axis cs:6,89.681840463467)
--(axis cs:7,139.679862935734)
--(axis cs:8,189.108736075865)
--(axis cs:9,40.3412269657519)
--(axis cs:10,68.5405581197068)
--(axis cs:11,88.9746569333947)
--(axis cs:12,102.526435107831)
--(axis cs:13,114.55600527572)
--(axis cs:14,125.367172949184)
--(axis cs:15,108.547696084017)
--(axis cs:16,117.299793389312)
--(axis cs:17,104.76420497636)
--(axis cs:18,99.9889739545574)
--(axis cs:19,116.773397484673)
--(axis cs:20,114.742126712369)
--(axis cs:21,124.299816177092)
--(axis cs:22,134.325447072958)
--(axis cs:23,126.615673863364)
--(axis cs:24,131.169527546422)
--(axis cs:25,132.452356449491)
--(axis cs:26,131.287994413408)
--(axis cs:27,127.946521560288)
--(axis cs:28,131.389053281581)
--(axis cs:29,125.71546665095)
--(axis cs:30,124.301182456051)
--(axis cs:31,126.605538933535)
--(axis cs:32,121.588181320109)
--(axis cs:33,127.278393304314)
--(axis cs:34,105.615236889488)
--(axis cs:35,107.950607389397)
--(axis cs:36,97.2925507079997)
--(axis cs:37,108.784325194055)
--(axis cs:38,74.6200336592448)
--(axis cs:39,77.7328105293221)
--(axis cs:40,133.690472554455)
--(axis cs:41,121.783958939276)
--(axis cs:42,131.498588056425)
--(axis cs:43,122.64901996408)
--(axis cs:44,145.765920089397)
--(axis cs:45,149.835854928937)
--(axis cs:46,156.533663834966)
--(axis cs:47,163.197903610009)
--(axis cs:48,165.98924855477)
--(axis cs:49,177.442336217765)
--(axis cs:50,161.514044698153)
--(axis cs:51,164.062671894874)
--(axis cs:52,166.681189941476)
--(axis cs:53,164.820368243246)
--(axis cs:54,144.217803939452)
--(axis cs:55,101.618599234376)
--(axis cs:56,108.227754403959)
--(axis cs:57,125.623294031879)
--(axis cs:58,99.4805912319884)
--(axis cs:59,90.9922955039038)
--(axis cs:60,100.067426477106)
--(axis cs:61,115.295006280823)
--(axis cs:62,143.603130188625)
--(axis cs:63,143.495565226323)
--(axis cs:64,144.232482389977)
--(axis cs:65,167.919858323579)
--(axis cs:66,179.913103875672)
--(axis cs:67,219.187239096912)
--(axis cs:68,220.508222522711)
--(axis cs:69,239.006517527893)
--(axis cs:70,228.458752466443)
--(axis cs:71,206.312668306283)
--(axis cs:72,197.602496917819)
--(axis cs:73,190.290225684462)
--(axis cs:74,192.325091401043)
--(axis cs:75,197.87260952242)
--(axis cs:76,170.156252640539)
--(axis cs:77,-31.6603388455954)
--(axis cs:78,206.187617285848)
--(axis cs:79,217.212106227373)
--(axis cs:79,369.187893772627)
--(axis cs:79,369.187893772627)
--(axis cs:78,335.412382714152)
--(axis cs:77,807.660338845595)
--(axis cs:76,421.643747359461)
--(axis cs:75,369.12739047758)
--(axis cs:74,363.274908598957)
--(axis cs:73,359.109774315538)
--(axis cs:72,357.797503082181)
--(axis cs:71,385.487331693717)
--(axis cs:70,411.541247533557)
--(axis cs:69,435.393482472107)
--(axis cs:68,445.491777477289)
--(axis cs:67,419.812760903088)
--(axis cs:66,420.286896124328)
--(axis cs:65,405.080141676421)
--(axis cs:64,424.967517610023)
--(axis cs:63,398.304434773677)
--(axis cs:62,386.396869811375)
--(axis cs:61,437.704993719177)
--(axis cs:60,439.332573522894)
--(axis cs:59,464.807704496096)
--(axis cs:58,421.519408768012)
--(axis cs:57,383.176705968121)
--(axis cs:56,407.972245596041)
--(axis cs:55,381.181400765624)
--(axis cs:54,326.182196060548)
--(axis cs:53,317.979631756754)
--(axis cs:52,306.518810058524)
--(axis cs:51,303.137328105126)
--(axis cs:50,273.285955301847)
--(axis cs:49,267.157663782235)
--(axis cs:48,259.01075144523)
--(axis cs:47,258.602096389991)
--(axis cs:46,250.666336165034)
--(axis cs:45,240.164145071063)
--(axis cs:44,251.434079910603)
--(axis cs:43,262.95098003592)
--(axis cs:42,251.901411943575)
--(axis cs:41,271.416041060724)
--(axis cs:40,239.709527445545)
--(axis cs:39,324.267189470678)
--(axis cs:38,324.179966340755)
--(axis cs:37,267.015674805945)
--(axis cs:36,246.307449292)
--(axis cs:35,210.849392610603)
--(axis cs:34,228.984763110512)
--(axis cs:33,212.921606695686)
--(axis cs:32,206.211818679891)
--(axis cs:31,191.594461066465)
--(axis cs:30,183.498817543949)
--(axis cs:29,175.48453334905)
--(axis cs:28,186.210946718419)
--(axis cs:27,181.853478439712)
--(axis cs:26,177.112005586591)
--(axis cs:25,175.947643550509)
--(axis cs:24,175.830472453578)
--(axis cs:23,169.984326136636)
--(axis cs:22,169.274552927042)
--(axis cs:21,178.700183822908)
--(axis cs:20,172.857873287631)
--(axis cs:19,169.426602515327)
--(axis cs:18,179.811026045443)
--(axis cs:17,177.43579502364)
--(axis cs:16,165.700206610688)
--(axis cs:15,181.252303915983)
--(axis cs:14,180.232827050816)
--(axis cs:13,178.24399472428)
--(axis cs:12,165.673564892169)
--(axis cs:11,160.025343066605)
--(axis cs:10,146.659441880293)
--(axis cs:9,248.658773034248)
--(axis cs:8,309.291263924135)
--(axis cs:7,209.720137064266)
--(axis cs:6,145.318159536533)
--(axis cs:5,84.8437304038987)
--(axis cs:4,64.4798069952578)
--(axis cs:3,36.1133676975115)
--(axis cs:2,25.4522720568516)
--(axis cs:1,20.237602458033)
--(axis cs:0,11.3518284528683)
--cycle;

\addplot [semithick, color0]
table {%
0 4
1 7.1
2 7.4
3 13.5
4 14.1
5 15.2
6 23.3
7 24.4
8 37.1
9 52.2
10 67.1
11 80.9
12 108.5
13 129.1
14 93.5
15 62.1
16 52.7
17 58.9
18 59.2
19 59.8
20 61
21 53.3
22 60.5
23 55.7
24 58
25 53.4
26 51.5
27 54.2
28 52.3
29 54.7
30 51.7
31 54.9
32 51.4
33 56.4
34 50.1
35 49.4
36 49
37 50.1
38 47
39 46.7
40 47
41 43.2
42 49.1
43 47.4
44 44.3
45 46.9
46 46.7
47 40.6
48 42.8
49 41.2
50 43.9
51 42.5
52 47.1
53 40.4
54 43.4
55 44.9
56 42.9
57 41.7
58 46.4
59 41.9
60 47.1
61 46.7
62 45.9
63 44.4
64 43.1
65 42.8
66 49.1
67 48.1
68 46.6
69 46
70 45.6
71 47.9
72 52.3
73 49.7
74 52.2
75 53.6
76 54.8
77 55.7
78 56.8
79 54
};
\addlegendentry{0.6 * ¦Â0}
\addplot [semithick, color1]
table {%
0 6.7
1 13.9
2 16.7
3 20.2
4 26.7
5 38.2
6 59.7
7 85.5
8 121.6
9 168.1
10 194.9
11 81.5
12 85.7
13 101.6
14 111.4
15 113.7
16 113.9
17 114.2
18 109.6
19 112.9
20 109.3
21 100.7
22 104.5
23 101.2
24 97.1
25 97
26 100.7
27 103.4
28 103.3
29 106.4
30 103.4
31 102.4
32 97
33 103.2
34 111
35 102
36 99.3
37 109.5
38 104.4
39 102.1
40 103.9
41 102.4
42 103.4
43 104.1
44 102.1
45 101
46 100.8
47 97.2
48 105.6
49 96.7
50 97.1
51 95.4
52 92.5
53 98.4
54 97.5
55 92
56 96
57 95.9
58 91.3
59 95.9
60 100.9
61 95.4
62 103.8
63 100
64 100.6
65 103.8
66 103.5
67 107
68 101.5
69 106.9
70 108.5
71 104.6
72 101.4
73 110.7
74 111.2
75 111
76 114.6
77 110.3
78 119
79 125.7
};
\addlegendentry{¦Â0}
\addplot [semithick, color2]
table {%
0 9.3
1 14.9
2 21.6
3 29
4 47.9
5 67.9
6 117.5
7 174.7
8 249.2
9 144.5
10 107.6
11 124.5
12 134.1
13 146.4
14 152.8
15 144.9
16 141.5
17 141.1
18 139.9
19 143.1
20 143.8
21 151.5
22 151.8
23 148.3
24 153.5
25 154.2
26 154.2
27 154.9
28 158.8
29 150.6
30 153.9
31 159.1
32 163.9
33 170.1
34 167.3
35 159.4
36 171.8
37 187.9
38 199.4
39 201
40 186.7
41 196.6
42 191.7
43 192.8
44 198.6
45 195
46 203.6
47 210.9
48 212.5
49 222.3
50 217.4
51 233.6
52 236.6
53 241.4
54 235.2
55 241.4
56 258.1
57 254.4
58 260.5
59 277.9
60 269.7
61 276.5
62 265
63 270.9
64 284.6
65 286.5
66 300.1
67 319.5
68 333
69 337.2
70 320
71 295.9
72 277.7
73 274.7
74 277.8
75 283.5
76 295.9
77 388
78 270.8
79 293.2
};
\addlegendentry{1.4 * ¦Â0}
\end{axis}

\end{tikzpicture}


==> pic/new198/new_infection_prop.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.862745098039216,0.0784313725490196,0.235294117647059}
\definecolor{color1}{rgb}{1,0.270588235294118,0}
\definecolor{color2}{rgb}{1,0.752941176470588,0.796078431372549}
\definecolor{color3}{rgb}{1,1,0}
\definecolor{color4}{rgb}{0.501960784313725,0,0.501960784313725}
\definecolor{color5}{rgb}{1,0.627450980392157,0.47843137254902}
\definecolor{color6}{rgb}{0.854901960784314,0.43921568627451,0.83921568627451}
\definecolor{color7}{rgb}{1,0,1}
\definecolor{color8}{rgb}{0.274509803921569,0.509803921568627,0.705882352941177}

\begin{axis}[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=white!89.8039215686275!black,inner xsep=0.1pt, inner ysep=-2.5pt, row sep=-4.5pt,at={(2.5,1.97)},ultra thin},
height=1.1in,width=0.2\linewidth,
font=\fontsize{1}{1.2}\selectfont,
tick align=outside,
tick pos=left,
title={new infection prop},
x grid style={white},
xlabel={step},
xmajorgrids,
xmin=-3.95, xmax=82.95,
xtick style={color=white!33.3333333333333!black},
y grid style={white},
ylabel={newly\_infected},
ymajorgrids,
ymin=-4.33460818508693e-06, ymax=9.10267718868255e-05,
ytick style={color=white!33.3333333333333!black},
ytick={-2e-05,0,2e-05,4e-05,6e-05,8e-05,0.0001},
yticklabels={−2,0,2,4,6,8,10}
]
\addplot [color0]
table {%
0 8.41671492249889e-07
1 0
2 0
3 0
4 1.68334298449978e-06
5 3.36668596899956e-06
6 1.68334298449978e-06
7 5.05002895349933e-06
8 5.05002895349933e-06
9 1.34667438759982e-05
10 9.25838641474878e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 8.41671492249889e-07
32 8.41671492249889e-07
33 0
34 0
35 0
36 8.41671492249889e-07
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 8.41671492249889e-07
68 0
69 8.41671492249889e-07
70 0
71 0
72 1.68334298449978e-06
73 0
74 8.41671492249889e-07
75 8.41671492249889e-07
76 8.41671492249889e-07
77 0
78 0
79 8.41671492249889e-07
};
\addlegendentry{workplace}
\addplot [color1]
table {%
0 0
1 0
2 0
3 0
4 8.41671492249889e-07
5 8.41671492249889e-07
6 0
7 8.41671492249889e-07
8 8.41671492249889e-07
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{school}
\addplot [color2]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{hospital}
\addplot [color3]
table {%
0 1.68334298449978e-06
1 1.68334298449978e-06
2 1.68334298449978e-06
3 4.20835746124944e-06
4 5.89170044574922e-06
5 5.89170044574922e-06
6 9.25838641474878e-06
7 1.43084153682481e-05
8 2.35668017829969e-05
9 3.0300173720996e-05
10 3.87168886434949e-05
11 3.36668596899956e-05
12 4.29252461047443e-05
13 5.38669755039929e-05
14 6.0600347441992e-05
15 4.5450260581494e-05
16 3.95585601357448e-05
17 4.79752750582437e-05
18 3.53502026744953e-05
19 2.86168307364962e-05
20 2.02001158139973e-05
21 2.52501447674967e-05
22 2.02001158139973e-05
23 2.2725130290747e-05
24 3.11418452132459e-05
25 2.18834587984971e-05
26 1.59917583527479e-05
27 1.85167728294976e-05
28 1.68334298449978e-05
29 1.85167728294976e-05
30 1.85167728294976e-05
31 1.68334298449978e-05
32 1.85167728294976e-05
33 2.2725130290747e-05
34 1.85167728294976e-05
35 1.43084153682481e-05
36 1.68334298449978e-05
37 1.85167728294976e-05
38 1.85167728294976e-05
39 1.85167728294976e-05
40 2.2725130290747e-05
41 1.5150086860498e-05
42 2.10417873062472e-05
43 1.68334298449978e-05
44 1.68334298449978e-05
45 1.01000579069987e-05
46 1.26250723837483e-05
47 1.34667438759982e-05
48 1.5150086860498e-05
49 1.5150086860498e-05
50 1.5150086860498e-05
51 8.41671492249889e-06
52 8.41671492249889e-06
53 1.09417293992486e-05
54 1.17834008914984e-05
55 1.5150086860498e-05
56 1.34667438759982e-05
57 1.5150086860498e-05
58 6.73337193799911e-06
59 1.26250723837483e-05
60 1.26250723837483e-05
61 1.09417293992486e-05
62 9.25838641474878e-06
63 7.575043430249e-06
64 1.34667438759982e-05
65 1.93584443217474e-05
66 1.43084153682481e-05
67 1.34667438759982e-05
68 1.68334298449978e-05
69 1.68334298449978e-05
70 1.34667438759982e-05
71 8.41671492249889e-06
72 1.5150086860498e-05
73 1.43084153682481e-05
74 1.85167728294976e-05
75 1.59917583527479e-05
76 1.68334298449978e-05
77 1.76751013372477e-05
78 2.02001158139973e-05
79 2.18834587984971e-05
};
\addlegendentry{household}
\addplot [green!50.1960784313725!black]
table {%
0 0
1 0
2 0
3 8.41671492249889e-07
4 8.41671492249889e-07
5 8.41671492249889e-07
6 0
7 1.68334298449978e-06
8 1.68334298449978e-06
9 5.89170044574922e-06
10 4.20835746124944e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{stadium}
\addplot [blue]
table {%
0 0
1 8.41671492249889e-07
2 8.41671492249889e-07
3 0
4 0
5 0
6 0
7 0
8 2.52501447674967e-06
9 2.52501447674967e-06
10 5.89170044574922e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{cinema}
\addplot [color4]
table {%
0 0
1 0
2 0
3 0
4 1.68334298449978e-06
5 0
6 8.41671492249889e-07
7 0
8 8.41671492249889e-07
9 3.36668596899956e-06
10 1.68334298449978e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{theatre}
\addplot [color5]
table {%
0 0
1 0
2 8.41671492249889e-07
3 0
4 0
5 8.41671492249889e-07
6 0
7 0
8 0
9 1.68334298449978e-06
10 5.05002895349933e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{library}
\addplot [red!50.1960784313725!black]
table {%
0 0
1 0
2 8.41671492249889e-07
3 0
4 0
5 0
6 0
7 8.41671492249889e-07
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{museum}
\addplot [black]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 8.41671492249889e-07
7 8.41671492249889e-07
8 8.41671492249889e-07
9 8.41671492249889e-07
10 3.36668596899956e-06
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
};
\addlegendentry{gym}
\addplot [white!50.1960784313725!black]
table {%
0 8.41671492249889e-07
1 0
2 1.68334298449978e-06
3 0
4 1.68334298449978e-06
5 4.20835746124944e-06
6 8.41671492249889e-07
7 1.43084153682481e-05
8 2.52501447674967e-06
9 4.20835746124944e-06
10 2.18834587984971e-05
11 6.73337193799911e-06
12 5.89170044574922e-06
13 9.25838641474878e-06
14 1.68334298449978e-05
15 1.01000579069987e-05
16 8.41671492249889e-06
17 1.01000579069987e-05
18 6.73337193799911e-06
19 6.73337193799911e-06
20 1.59917583527479e-05
21 1.5150086860498e-05
22 1.68334298449978e-05
23 1.26250723837483e-05
24 1.17834008914984e-05
25 1.01000579069987e-05
26 1.09417293992486e-05
27 8.41671492249889e-06
28 9.25838641474878e-06
29 8.41671492249889e-06
30 4.20835746124944e-06
31 1.01000579069987e-05
32 1.17834008914984e-05
33 3.36668596899956e-06
34 9.25838641474878e-06
35 9.25838641474878e-06
36 4.20835746124944e-06
37 1.01000579069987e-05
38 5.89170044574922e-06
39 5.05002895349933e-06
40 1.09417293992486e-05
41 7.575043430249e-06
42 4.20835746124944e-06
43 8.41671492249889e-06
44 7.575043430249e-06
45 6.73337193799911e-06
46 3.36668596899956e-06
47 2.52501447674967e-06
48 3.36668596899956e-06
49 2.52501447674967e-06
50 5.89170044574922e-06
51 5.05002895349933e-06
52 5.05002895349933e-06
53 3.36668596899956e-06
54 1.26250723837483e-05
55 5.05002895349933e-06
56 6.73337193799911e-06
57 5.05002895349933e-06
58 1.01000579069987e-05
59 5.05002895349933e-06
60 6.73337193799911e-06
61 5.89170044574922e-06
62 6.73337193799911e-06
63 1.01000579069987e-05
64 7.575043430249e-06
65 5.05002895349933e-06
66 1.17834008914984e-05
67 3.36668596899956e-06
68 6.73337193799911e-06
69 9.25838641474878e-06
70 6.73337193799911e-06
71 3.36668596899956e-06
72 9.25838641474878e-06
73 4.20835746124944e-06
74 9.25838641474878e-06
75 7.575043430249e-06
76 8.41671492249889e-06
77 6.73337193799911e-06
78 1.26250723837483e-05
79 6.73337193799911e-06
};
\addlegendentry{retail}
\addplot [color6]
table {%
0 0
1 0
2 8.41671492249889e-07
3 1.68334298449978e-06
4 8.41671492249889e-07
5 8.41671492249889e-07
6 0
7 2.52501447674967e-06
8 2.52501447674967e-06
9 4.20835746124944e-06
10 4.20835746124944e-06
11 0
12 0
13 0
14 0
15 8.41671492249889e-07
16 8.41671492249889e-07
17 0
18 8.41671492249889e-07
19 8.41671492249889e-07
20 8.41671492249889e-07
21 1.68334298449978e-06
22 8.41671492249889e-07
23 0
24 8.41671492249889e-07
25 0
26 8.41671492249889e-07
27 0
28 8.41671492249889e-07
29 0
30 0
31 1.68334298449978e-06
32 8.41671492249889e-07
33 1.68334298449978e-06
34 0
35 8.41671492249889e-07
36 8.41671492249889e-07
37 0
38 0
39 8.41671492249889e-07
40 2.52501447674967e-06
41 0
42 8.41671492249889e-07
43 0
44 0
45 8.41671492249889e-07
46 8.41671492249889e-07
47 8.41671492249889e-07
48 0
49 1.68334298449978e-06
50 0
51 0
52 0
53 0
54 8.41671492249889e-07
55 0
56 8.41671492249889e-07
57 0
58 0
59 0
60 0
61 0
62 8.41671492249889e-07
63 0
64 0
65 0
66 8.41671492249889e-07
67 0
68 0
69 1.68334298449978e-06
70 0
71 0
72 8.41671492249889e-07
73 8.41671492249889e-07
74 8.41671492249889e-07
75 8.41671492249889e-07
76 0
77 0
78 0
79 1.68334298449978e-06
};
\addlegendentry{community}
\addplot [color7]
table {%
0 3.36668596899956e-06
1 4.20835746124944e-06
2 2.52501447674967e-06
3 3.36668596899956e-06
4 1.17834008914984e-05
5 2.02001158139973e-05
6 1.93584443217474e-05
7 1.68334298449978e-05
8 4.62919320737439e-05
9 4.04002316279947e-05
10 8.66921637017386e-05
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 8.41671492249889e-07
65 0
66 0
67 8.41671492249889e-07
68 0
69 0
70 8.41671492249889e-07
71 8.41671492249889e-07
72 0
73 8.41671492249889e-07
74 0
75 0
76 0
77 0
78 0
79 8.41671492249889e-07
};
\addlegendentry{restaurant}
\addplot [color8]
table {%
0 0
1 0
2 1.68334298449978e-06
3 1.68334298449978e-06
4 3.36668596899956e-06
5 3.36668596899956e-06
6 5.89170044574922e-06
7 3.36668596899956e-06
8 7.575043430249e-06
9 1.17834008914984e-05
10 2.18834587984971e-05
11 7.575043430249e-06
12 8.41671492249889e-06
13 5.89170044574922e-06
14 9.25838641474878e-06
15 1.17834008914984e-05
16 5.89170044574922e-06
17 1.26250723837483e-05
18 3.36668596899956e-06
19 5.89170044574922e-06
20 4.20835746124944e-06
21 1.01000579069987e-05
22 5.89170044574922e-06
23 8.41671492249889e-06
24 3.36668596899956e-06
25 7.575043430249e-06
26 9.25838641474878e-06
27 7.575043430249e-06
28 1.09417293992486e-05
29 6.73337193799911e-06
30 6.73337193799911e-06
31 5.89170044574922e-06
32 1.09417293992486e-05
33 8.41671492249889e-06
34 7.575043430249e-06
35 7.575043430249e-06
36 5.89170044574922e-06
37 7.575043430249e-06
38 7.575043430249e-06
39 5.05002895349933e-06
40 9.25838641474878e-06
41 6.73337193799911e-06
42 5.05002895349933e-06
43 8.41671492249889e-06
44 4.20835746124944e-06
45 9.25838641474878e-06
46 6.73337193799911e-06
47 2.52501447674967e-06
48 4.20835746124944e-06
49 5.89170044574922e-06
50 4.20835746124944e-06
51 1.68334298449978e-06
52 6.73337193799911e-06
53 1.68334298449978e-06
54 7.575043430249e-06
55 3.36668596899956e-06
56 8.41671492249889e-07
57 5.89170044574922e-06
58 4.20835746124944e-06
59 9.25838641474878e-06
60 8.41671492249889e-06
61 5.05002895349933e-06
62 1.09417293992486e-05
63 3.36668596899956e-06
64 9.25838641474878e-06
65 2.52501447674967e-06
66 7.575043430249e-06
67 6.73337193799911e-06
68 5.05002895349933e-06
69 2.52501447674967e-06
70 4.20835746124944e-06
71 5.89170044574922e-06
72 7.575043430249e-06
73 4.20835746124944e-06
74 7.575043430249e-06
75 6.73337193799911e-06
76 3.36668596899956e-06
77 8.41671492249889e-06
78 7.575043430249e-06
79 5.89170044574922e-06
};
\addlegendentry{supermarket}
\end{axis}

\end{tikzpicture}

